W2VLDA: Almost Unsupervised System for Aspect Based Sentiment Analysis

With the increase of online customer opinions in specialised websites and social networks, the necessity of automatic systems to help to organise and classify customer reviews by domain-specific aspect/categories and sentiment polarity is more important than ever. Supervised approaches to Aspect Based Sentiment Analysis obtain good results for the domain/language their are trained on, but having manually labelled data for training supervised systems for all domains and languages are usually very costly and time consuming. In this work we describe W2VLDA, an almost unsupervised system based on topic modelling, that combined with some other unsupervised methods and a minimal configuration, performs aspect/category classifiation, aspect-terms/opinion-words separation and sentiment polarity classification for any given domain and language. We evaluate the performance of the aspect and sentiment classification in the multilingual SemEval 2016 task 5 (ABSA) dataset. We show competitive results for several languages (English, Spanish, French and Dutch) and domains (hotels, restaurants, electronic-devices).

==> tab_sentence_examples.tex <==
% Table generated by Excel2LaTeX from sheet 'Hoja2'
\begin{table}[htbp]
\footnotesize
  \centering
    \begin{tabular}{|p{2.2cm}|p{1.5cm}|p{10cm}|}
    \hline
    Language:Domain & \multicolumn{1}{p{2cm}|}{Domain Topic} & Examples of sentences with high posterior probability for different topics\bigstrut\\
    \hline
    \hline
    \multicolumn{1}{|p{2cm}|}{\multirow{3}[6]{*}{\parbox{2.2cm}{English:\\ restaurant reviews}}} & Food  & {\parbox{10cm}{Appetizer was grilled pizza dough topped with fig jam, prosciutto, arugula, cherry tomatoes...\\
Four of us enjoyed sizziling rice seafood soup, the most savory garlic string beans.}} \bigstrut\\
\cline{2-3}          & Service & {\parbox{10cm}{Seated promptly, waiter arrived at 6:10 brought us our drink order 6:15.\\
Bartenders are friendly and quick to be helpful }}\bigstrut\\
\cline{2-3}          & Ambiance & {\parbox{10cm}{The atmosphere as a restaurant though is very nice: cute decor, quieter, and dim lighting...\\
The ambiance of the restaurant is very nice, the decor and lighting set a great atmosphere}} \bigstrut\\
    \hline
    \hline
    \multicolumn{1}{|p{2cm}|}{\multirow{3}[6]{*}{\parbox{2.2cm}{Spanish:\\ restaurant reviews}}} & Food  & {\parbox{10cm}{Probamos las croquetas melosas de jam\'on, milhoja de tomate y mozzarella con salsa de miel.\\
Pat\'e de perdiz, tartar de bonito, steak tartar, pat\'e de cabracho, brocheta de pollo y postres}} \bigstrut\\
\cline{2-3}          & Service & {\parbox{10cm}{El servicio a los clientes deja bastante que desear\\
El trato es magn\'ifico, camareros muy simp\'aticos y amables, un trato educado y exquisito}} \bigstrut\\
\cline{2-3}          & Ambiance & {\parbox{10cm}{ Cena agradable en un lugar de ambiente tranquilo, cosmopolita, con buena m\'usica\\
 El local es feo decorado como un bar de carretera en EEUU o un autob\'us}} \bigstrut\\
    \hline
    \hline
    \multirow{3}[6]{*}{\parbox{2.2cm}{French:\\ hotel reviews}} & Staff & {\parbox{10cm}{Service de qualit\`e et personnel extr\^emement agreable, aux petits soins, disponible et serviable!\\
Le personnel est r\`eactif, serviable, disponible, toujours pr\^et \`a r\`epondre aux attentes des clients.}} \bigstrut\\
\cline{2-3}          & Ambiance & {\parbox{10cm}{L’hotel est une attraction en soi, il y a un adventure park a l’interieur, on se croirait a disneyland.\\
Le b\^atiment a un certain charme, certaines tapisseries sont d\`efra\^ichies, se sent londonien}} \bigstrut\\
\cline{2-3}          & Location & {\parbox{10cm}{A 5 minutes \`a pied de buckingham palace et saint james park , 10 \`a 15 minutes de big ben.\\
Hotel \`a 15 min de la gare \`a pied, à 15 min d'oxford street, \`a 40 min du centre ville \`a pied.}} \bigstrut\\
    \hline
    \end{tabular}%
      \caption{Some examples of sentences with the highest posterior probability for several topics, domains and languages.}
  \label{tab:topic_sentences_example}%
\end{table}%

==> tab_topic_word_examples.tex <==
% Table generated by Excel2LaTeX from sheet 'Hoja1'
\begin{table}[htbp]
\scriptsize
  \centering
    \begin{tabular}{|p{2.4cm}|p{1.5cm}|p{2.8cm}|p{2.8cm}|p{2.8cm}|}
    \hline
    Language:Domain & \multicolumn{1}{c|}{Domain topic} & \multicolumn{1}{c|}{Aspect-terms} & \multicolumn{1}{c|}{Positive words} & \multicolumn{1}{c|}{Negative words} \bigstrut\\
    \hline
    \hline
    \multirow{3}[6]{*}{\parbox{2.4cm}{English:\\ restaurant reviews}} &\vspace{.02\baselineskip} Food  & \vspace{.02\baselineskip} chicken, beef, pork, tuna, egg, onions, shrimp, curry & \vspace{.02\baselineskip} moist, goat, smoked, seared, roasted, red, crispy, tender & \vspace{.02\baselineskip} undercooked, dry, drenched, overcooked, soggy, chewy \bigstrut\\
\cline{2-5}          & \vspace{.02\baselineskip} Service & \vspace{.02\baselineskip} staff, workers, employees, chefs, hostess, manager, owner & \vspace{.02\baselineskip} helpful, polite, knowledgeable, efficient, prompt, attentive & \vspace{.02\baselineskip} inattentive, rude, unfriendly, wearing, making, packed \bigstrut\\
\cline{2-5}          & \vspace{.02\baselineskip} Ambiance & \vspace{.02\baselineskip} lighting, wall, interior, vibe, concept, ceilings, setting & \vspace{.02\baselineskip} modern, beautiful, chic, nice, trendy, cozy, elegant & \vspace{.02\baselineskip} bad, loud, uninspired, expensive, big, noisy, dark, cramped \bigstrut\\
    \hline
    \hline
    \multirow{3}[6]{*}{\parbox{2.4cm}{Spanish:\\ restaurant reviews}} & \vspace{.02\baselineskip} Food  & \vspace{.02\baselineskip} crema, tartar, ensaladas, sopa, brasa, patatas, salsas, alcachofas & \vspace{.02\baselineskip} caprese, sublime, destacar, casera, tierna, trufada, ahumada & \vspace{.02\baselineskip} aguada, mojar, congeladas, quemadas, fritos, rancias, reseco \bigstrut\\
\cline{2-5}          &\vspace{.02\baselineskip} Service &\vspace{.02\baselineskip} camareros, camarero, maitre, due\~no, encargado, metre &\vspace{.02\baselineskip} eficiente, eficaz, atentos, correcta, cercano, diligente & \vspace{.02\baselineskip}lento, p\'esimo, desagradable, prepotente, maleducado \bigstrut\\
\cline{2-5}          & \vspace{.02\baselineskip}Ambiance & \vspace{.02\baselineskip} toques, atm\'osfera, material, mobiliario, bancos, modernidad &  \vspace{.02\baselineskip}tranquilo, relajado, c\'alido,  buena, amplio, luminoso, precioso, & \vspace{.02\baselineskip} cutre, insoportable, peque\~no, tanta, oscuro, poca, normalita \bigstrut\\
    \hline
    \hline
    \multirow{3}[6]{*}{\parbox{2.4cm}{French:\\ hotel reviews}} &\vspace{.02\baselineskip} Food  &\vspace{.02\baselineskip} nourriture, sauce, produits, p\^ate, bouffe, saveur, risotto & \vspace{.02\baselineskip} raisonnable, michelin,  excellents, merveilleuse, veritable, superbe & \vspace{.02\baselineskip} correcte,  cuit, idem, passable, excessif, moleculaire, difficile \bigstrut\\
\cline{2-5}          & \vspace{.02\baselineskip}Staff & \vspace{.02\baselineskip} personnel, \`ecoute, staff, gentillesse, concierge, membres & \vspace{.02\baselineskip} sympathique, attentionn\'e, efficace, compètent, professionnel & \vspace{.02\baselineskip} d\`eplorable,  antipathique, d\`ebord\`e, distant, constamment \bigstrut\\
\cline{2-5}          & \vspace{.02\baselineskip} Ambiance & \vspace{.02\baselineskip} impression, couloirs, odeurs, personnages, hiver, escaliers & \vspace{.02\baselineskip} vieillissant, grand, r\`enov\`e, boone, typiquement, cosy, agr\`eablement & \vspace{.02\baselineskip} froide, v\`etuste, forte, incendie, bruyants, inexistante, compl\`ete \bigstrut\\
    \hline
    \hline
    \multirow{3}[6]{*}{\parbox{2.4cm}{English:\\ electronic devices reviews}} & Warranty & warranty, support, repair, service, answer, center, policy & worked, lucky, owned, big, exchange, extended, longer & called, contact, broken, faulty, defective, expired, worthless \bigstrut\\
\cline{2-5}          & Design & plastic, wheel, style, handle, pocket, design, exterior, wheels & adjustable, clean, good, versatile, attractive, lightweight, stylish & ugly, odd, awkward, tight, felt, weird, cute, stupid, flimsy \bigstrut\\
\cline{2-5}          & Price & money, store, item, bucks, price, regret, deal, gift & paying, reasonable, penny, worth, delivered, stars, inexpensive,  & disappointed, paid, cheaper, skeptical, pricey, overpriced \bigstrut\\
    \hline
    \end{tabular}%
    \caption{Resulting topic words distributions for several languages and domains. The topics are automatically split into three different word distributions: topic aspect terms, topic positive words and topic negative words.}
  \label{tab:topic_words_example}%
\end{table}%

